Scattering Loss in Precision Metrology due to Mirror Roughness

Optical losses degrade the sensitivity of laser interferometric instruments. They reduce the number of signal photons and introduce technical noise associated with diffuse light. In quantum-enhanced metrology, they break the entanglement between correlated photons. Such decoherence is one of the primary obstacles in achieving high levels of quantum noise reduction in precision metrology. In this work, we compare direct measurements of cavity and mirror losses in the Caltech 40m gravitational-wave detector prototype interferometer with numerical estimates obtained from semi-analytic intra-cavity wavefront simulations using mirror surface profile maps. We show a unified approach to estimating the total loss in optical cavities (such as the LIGO gravitational detectors) that will lead towards the engineering of systems with minimum decoherence for quantum-enhanced precision metrology.

==> Comparison_Of_Theory_And_Measurement.tex <==
\section{Comparison of measurements}
\label{s:Comparison}
\Yeh{Yehonathan, Tega}
In this paper we employed several direct (DC Reflection, Power recycling gain) and indirect (Phase maps, total integrating sphere, scattering measurements) loss measurement techniques. We have shown that the direct and indirect techniques are consistent within themselves. In table~\ref{tab:paper_results} we summarize those results.
\begin{center}
	\begin{table}
		\renewcommand{\arraystretch}{2}
		\begin{tabular}{| @{\hspace{0.5cm}} c @{\hspace{0.5cm}}| @{\hspace{0.5cm}}c @{\hspace{0.5cm}}| @{\hspace{0.5cm}}c@{\hspace{0.5cm}} |}
			\hline
			Parameter &Nominal Value & Uncertainty\\ 
			\hline
			DC Reflection measurement after cleaning & 28 ppm & $\pm$ 6 ppm\\
			\hline
			Phase map loss & 6 ppm & $\pm$ 2 ppm\\
			\hline
			ETM CCD measurement inferred loss & 19 ppm & $\pm$ 3 ppm\\
			\hline
			TIS measurement ($\SI{1}{\degree}<\theta<\SI{75}{\degree})$& 9.3 ppm & $\pm$ 1.2 ppm \\
			\hline
			BRDF measurement inferred loss &  & \\
			\hline
		\end{tabular}
		\caption{Summary of the experimental results of this paper.}
		\label{tab:paper_results}
	\end{table}
\end{center}

\newpage
%\begin{figure}[h!]
%\centering\includegraphics[width=0.8\columnwidth]{lossesV2.png}
%\caption{Comparison of measured losses with expected loss level}
%\end{figure}

